Assessing the Impact of Interface Vulnerabilities in Compartmentalized Software

Least-privilege separation decomposes applications into compartments limited to accessing only what they need. When compartmentalizing existing software, many approaches neglect securing the new inter-compartment interfaces, although what used to be a function call from/to a trusted component is now potentially a targeted attack from a malicious compartment. This results in an entire class of security bugs: Compartment Interface Vulnerabilities (CIVs). This paper provides an in-depth study of CIVs. We taxonomize these issues and show that they affect all known compartmentalization approaches. We propose ConfFuzz, an in-memory fuzzer specialized to detect CIVs at possible compartment boundaries. We apply ConfFuzz to a set of 25 popular applications and 36 possible compartment APIs, to uncover a wide data-set of 629 vulnerabilities. We systematically study these issues, and extract numerous insights on the prevalence of CIVs, their causes, impact, and the complexity to address them. We stress the critical importance of CIVs in compartmentalization approaches, demonstrating an attack to extract isolated keys in OpenSSL and uncovering a decade-old vulnerability in sudo. We show, among others, that not all interfaces are affected in the same way, that API size is uncorrelated with CIV prevalence, and that addressing interface vulnerabilities goes beyond writing simple checks. We conclude the paper with guidelines for CIV-aware compartment interface design, and appeal for more research towards systematic CIV detection and mitigation.

==> Makefile <==
TARGET=paper
SRC= 00-abstract.tex 03-interface-vulnerabilities.tex \
	 04-design-and-implementation.tex 06-discussion.tex 08-conclusion.tex \
	 01-introduction.tex 02-motivation.tex 05-evaluation.tex \
	 07-related-works.tex paper.tex

dvi: all

all:
	pdflatex --draftmode -shell-escape $(TARGET)
	bibtex $(TARGET)
	pdflatex -shell-escape $(TARGET)
	pdflatex -shell-escape $(TARGET)

show: all
	evince $(TARGET).pdf

spellcheck:
	$(foreach f,$(SRC), aspell -l EN_US -t -c $(f) -p ./.aspell.txt;)


# Diff target for revision modifications
# Make sure you modify latexdiff as described here:
# https://tex.stackexchange.com/a/579662
latexdiff:
	git latexdiff --exclude-textcmd="paragraph" \
		--config='PICTUREENV=(?:picture|DIFnomarkup|listing|lstlisting)[\w\d*@]*' \
		--main paper.tex \
		-o latexdiff.pdf \
		b85746c69b70ba435b93a277ff1b7ecb44696f18

cover-letter:
	make -C submissions/ndss-revision-cover-letter

supplementary-materials: cover-letter latexdiff
	pdfunite submissions/ndss-revision-cover-letter/ndss-117-cover-letter.pdf latexdiff.pdf $@.pdf

clean:
	rm -rf *.aux *.log *.toc *.blg *.out *.pygtex *.pygstyle minted-cache

superclean: clean
	rm -rf $(TARGET).pdf latexdiff.pdf

